FreshLLMs: Refreshing Large Language Models with Search Engine Augmentation

Most large language models (LLMs) are trained once and never updated; thus, they lack the ability to dynamically adapt to our ever-changing world. In this work, we perform a detailed study of the factuality of LLM-generated text in the context of answering questions that test current world knowledge. Specifically, we introduce FreshQA, a novel dynamic QA benchmark encompassing a diverse range of question and answer types, including questions that require fast-changing world knowledge as well as questions with false premises that need to be debunked. We benchmark a diverse array of both closed and open-source LLMs under a two-mode evaluation procedure that allows us to measure both correctness and hallucination. Through human evaluations involving more than 50K judgments, we shed light on limitations of these models and demonstrate significant room for improvement: for instance, all models (regardless of model size) struggle on questions that involve fast-changing knowledge and false premises. Motivated by these results, we present FreshPrompt, a simple few-shot prompting method that substantially boosts the performance of an LLM on FreshQA by incorporating relevant and up-to-date information retrieved from a search engine into the prompt. Our experiments show that FreshPrompt outperforms both competing search engine-augmented prompting methods such as Self-Ask (Press et al., 2022) as well as commercial systems such as Perplexity.AI. Further analysis of FreshPrompt reveals that both the number of retrieved evidences and their order play a key role in influencing the correctness of LLM-generated answers. Additionally, instructing the LLM to generate concise and direct answers helps reduce hallucination compared to encouraging more verbose answers. To facilitate future work, we release FreshQA at github.com/freshllms/freshqa and commit to updating it at regular intervals.

==> pubapprove_reviews.tex <==
============================== Reviewer 1 ==============================
This paper introduces a new benchmark FreshQA to evaluate language models' ability to provide up-to-date information, and a prompting methodology to incorporate search results for higher accuracy.

Here are some suggestions for improvement:

1. Where do FreshQA questions come from, hand-written? Is there any consideration on the coverage of its topics?

2. Relaxed vs strict: do they differ at factuality (i.e. relaxed means the final answer is correct but the intermediate steps may be wrong), or at beauty / easy to understand (since the model response to Figure 2 ID 4 "Which language has the third largest population by number of native speakers" seems factually correct)? Is there a metric / scoring function to determine whether an answer is correct in either the relaxed or strict setting? If so, the rubric would be easier for other people to adopt, and the FreshQA benchmark would be easier to maintain.

3. Beyond Figure 4 that shows the search results, an intuitive diagram or an example prompt of how search results are incorporated into the prompt (and thus used to do in-context learning) is needed. I assume the authors will add this in the revision.

4. Beyond FreshQA, is (a subset of) truthfulQA also something worth benchmarking on?

Despite these suggestions, the paper is recommended for publication because:

1. The paper uses no proprietary model or data. All Google models in use have been announced in previous papers / blog posts, and the evaluations are based on a new benchmark dataset solely proposed by the authors here.

2. The paper is scientifically interesting as it introduces a new benchmark to evaluate different models' ability to provide up-to-date answers.

3. Given that using search results to augment prompting isn't a new direction, publishing this work won’t help accelerate competing teams.

============================== Reviewer 2 ==============================
This work studies LLM factuality regarding queries that require up-to-date knowledge. First, it introduces FreshQA benchmark that contains factuality questions that are based on knowledge ranging from never-changing to fast-changing, as well as false premise questions. The evaluation shows that without access to search results, none of the evaluated LLMs performs well on questions that require knowledge after 2022. Accordingly, they design a prompting method called SEAL to incorporate search information in the prompt, which significantly improves the performance.

From the research aspect, I feel that the scientific contribution of this work is mainly on providing a more systematic study of LLM factuality compared to prior work.

1. Despite that there have been a couple of existing benchmarks on QA based on real-time information, FreshQA provides more fine-grained categories (never-changing to fast-changing), as well as incorporating false premise questions.

2. Although prompting with augmented search results is also not new, this work presents a comprehensive evaluation on how the search results can be formatted, and how different implementations affect the performance.

Given that all evaluated models have been publicly announced, and the data and method also do not have competitive concerns, I think this work is good for publication.

Below are some questions/comments about the draft:

1. It is helpful to explain more clearly on why it is helpful to construct a new benchmark instead of evaluating on existing benchmarks that study relevant topics. If time allowed, it would be good to also evaluate on an existing benchmark like RealTimeQA.

2. The current description of SEAL is unclear. It would be good to give some sample prompts.

3. After reading Table 2 and the discussion, I still cannot understand why SEAL is significantly better than self-ask and Perplexity.AI. Since Perplexity.AI is black-box, it is fine if we do not have an explanation. But to my knowledge, the main difference between self-ask and SEAL is that self-ask includes question decomposition, while SEAL does not. If this is the case, why should question decomposition degrades the performance on both 1-hop and multi-hop questions? More explanation of SEAL implementation might help clarify this question, but currently it is confusing and needs more explanation.

4. Unless you have any extra source of information, publicly people do not have confirmed information on the true sizes of gpt-3.5-turbo, text-davinci-003 and Codex either.


